A machine learning based plasticity model using proper orthogonal decomposition

Data-driven material models have many advantages over classical numerical approaches, such as the direct utilization of experimental data and the possibility to improve performance of predictions when additional data is available. One approach to develop a data-driven material model is to use machine learning tools. These can be trained offline to fit an observed material behaviour and then be applied in online applications. However, learning and predicting history dependent material models, such as plasticity, is still challenging. In this work, a machine learning based material modelling framework is proposed for both elasticity and plasticity. The machine learning based hyperelasticity model is developed with the Feed forward Neural Network (FNN) directly whereas the machine learning based plasticity model is developed by using of a novel method called Proper Orthogonal Decomposition Feed forward Neural Network (PODFNN). In order to account for the loading history, the accumulated absolute strain is proposed to be the history variable of the plasticity model. Additionally, the strain-stress sequence data for plasticity is collected from different loading-unloading paths based on the concept of sequence for plasticity. By means of the POD, the multi-dimensional stress sequence is decoupled leading to independent one dimensional coefficient sequences. In this case, the neural network with multiple output is replaced by multiple independent neural networks each possessing a one-dimensional output, which leads to less training time and better training performance. To apply the machine learning based material model in finite element analysis, the tangent matrix is derived by the automatic symbolic differentiation tool AceGen. The effectiveness and generalization of the presented models are investigated by a series of numerical examples using both 2D and 3D finite element analysis.

==> Fig/MachineLearning.tex <==
\chapter{Machine Learning based Material Model \label{chap:ml}}
%
\section{Data-driven material modelling framework}
The phenomenological material model, such as the Johnson-Cook model, shows good performance for some simple loading conditions, such as the tension of the notched bar. However, it does not always close to the experimental results when the structure undergoes some complex deformations such as the shear dominated loadings. Thus the parameters of the material model needs to be calibrated further by conducting more experiments. In some cases, the material model has to be modified to account for more physical effects. To replace the classical material modelling approach, the data-driven material modelling approach is investigated in this section, which provides an alternative tool to narrow the gap between the data and the material modelling.

As shown in Fig.\ref{flowchart}, there are three steps in the material modelling framework: data collection, machine learning and testing in FEM analysis. As a direct description the material behaviour, the training data can be collected from the experiments and the simulations. Before collecting the training data, loading conditions have to be determined, which will suggest what kind of experiments or simulations does it need to be conducted. Depending on the problem, the training data usually has to be preprocessed by extracting the data from specific loading paths, scaling the data into specific range or data decomposition. The training data has to be as compact as possible to avoid additional training efforts. 

Then the artificial neural networks as a machine learning technology will be employed to learn the features or patterns existed in the training data. The type of neural networks, the architecture of the neural networks and the training algorithm will be selected according to the training performance. The machine learning based material model will then be build from trained neural networks. 

The following step is to test machine learning based material model by the finite element analysis. By deriving the material tangent, the machine learning based model can be incorporated into the FEM code. The performance of the machine learning based material model is evaluated by the benchmark tests in FEM. If the material model can not meet the accuracy requirement in FEM analysis, the improvements, such as supplementing additional data and improving the training accuracy, will be made until an acceptable training accuracy is achieved.\\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.8\columnwidth}
	\import{chap_MachineLearning/}{flowchart.pdf_tex}
	\caption{The data-driven material modelling framework}
	\label{flowchart}
\end{figure}

In this section, the machine learning based hyper-elasticity model is firstly developed by applying the feed forward neural networks. The performance of the  machine learning based hyper-elasticity model is evaluated by the numeral examples in FEM. Then, the data generation strategy for the plasticity model is proposed referring to the first step in the above framework. Finally, two machine learning based elasto-plasticity models are developed, one is based on the recurrent neural networks and another one is based on the feed forward neural networks together with the Proper Orthogonal Decomposition (POD). The loading history is recorded within the recurrent neural networks automatically, whereas the additional history variable is chosen to distinguish the loading history for the feed forward neural networks. In feed forward neural network based plasticity model, the stress sequences are represented by the Proper Orthogonal Decomposition (POD), which leads to a decoupled model composed of three independent feed forward neural networks. The tangent matrix is derived by a symbolic tool AceGen, thus the model is validated by the benchmark tests in Finite Element Analysis.

\section{Feed forward Neural Network (FNN) based hyper-elasticity}
\subsection{Feed forward neural network}
The feed forward neural network (FNN) is a fundamental network architecture in machine learning technology. The FNN is composed by several connected layers of artificial neurons and biases, where the data is feed into the input layer, then flows through all of the hidden layers and finally the prediction is given at the output layer, as shown in Fig. \ref{fnntrain}. Each neuron in one layer are connected with that in its adjacent layer through a weight $w$. In the prediction phase, the data flows in one way from the input layer to the output layer, therefore it is called feed forward neural network. However, in the training phase, the output data of neural network will be compared with the target data and then evaluated with the global error. The weights of the neural network will be updated by back propagating the gradient of the global error, which aims to minimize the global error.\\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.85\columnwidth}
	\import{chap_MachineLearning/}{fnntrain.pdf_tex}
	\caption{The FNN}
	\label{fnntrain}
\end{figure}
%more details see: https://de.mathworks.com/help/deeplearning/ug/neural-network-architectures.html?searchHighlight=sigmoid%20function%20neural%20network&s_tid=doc_srchtitle%

As the basic element of FNN, the artificial neurons in different layers are fully connected through the weight matrix $W$, which means the data output from one neuron will be multiplied with the weight before feeding into its connected neuron. At each neuron, the input data from all neurons of the previous layer will be summed and then feed into the activation function attached on this neuron, as shown in Fig.\ref{neuron}. A normal choice of the activation function is the sigmoid function:
\begin{align}
f_s(x)=\frac{2}{1+e^{-a(x-c)}}-1,
\end{align}
where $a$ and $c$ are the function parameters. The value of the parameters are assigned as: $a=2, c=0$ in this work. The plot of sigmoid function is depicted in Fig.\ref{sigmf}, where the sensitive region is located anti-symmetrical around the original point. For one neuron $j$ in layer $k$, the data from the neurons of previous layer $k-1$ are summed up firstly and then feed into the activation function. The output of the neuron $j$ in layer $k$ is 
\begin{align}
o_j^k=f_s\left( \sum_{i=1}^{N} w_{ij} o_i^{k-1}+b^{k-1} \right),
\end{align}
where $N$ is the number of neuron in the previous layer $k-1$, $w_{ij}$ is the weight in the connection between neuron $i$ and $j$, $o_i^{k-1}$ is the output of the neuron $i$ in layer $k-1$ whereas $b^{k-1}$ is the bias for this neuron.\\ 

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.5\columnwidth}
	\import{chap_MachineLearning/}{neuron.pdf_tex}
	\caption{The artificial neuron}
	\label{neuron}
\end{figure}

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.4\columnwidth}
	\import{chap_MachineLearning/}{sigmoidfun.pdf_tex}
	\caption{The sigmoid activation function}
	\label{sigmf}
\end{figure}
The specific architecture of the FNN, such as the number of layer and the number of neuron in each layer, has to be determined according to the complexity of the model. For the function fitting problem, only one hidden layer is usually enough. For the more complex problem, more than one hidden layers are required. However, there is no theoretical suggestion reported in literature for the chosen of neural network architecture, but the trail and error approach.
 
\subsection{Back propagation algorithm}
The weighs of the neural network will be initialised randomly once the architecture is built. The next step is to train the neural network by the given data set, where the weights will be updated to minimize the global error based on the back propagation algorithm. The global error, also named as loss function or network performance, is defined according to the difference of the network prediction and the target data. The mean squared error is usually applied as the loss function
\begin{align}
E(\boldsymbol{w})=\frac{1}{N} \sum_{i=1}^{N} \left[ o_i(\boldsymbol W)-t_i \right]^2=\frac{1}{N} \sum_{i=1}^{N}  e_i,
\end{align}
where $N$ is the number of the output, the $o_i$ is the $i$-th output, $\boldsymbol W$ is the weight matrix, and $t_i$ is the $i$-th target value. For a specific set of training data including the inputs and the outputs, the problem to minimize the loss function becomes the optimization problem, where the loss function can be seen as the objective function. To train the feed forward neural network, the gradient based algorithm has to be applied. Since the hidden layers are located parallel with the output layer, the so called back propagation technique will be used to compute the gradients in terms of the weights. Fig.\ref{bp} shows the connections of 3 neurons in the output and hidden layer in the FNN, where the partial derivative of global loss $E$ with respect to weight $w$ will be computed by back propagating the error from output layer to the hidden layers.\\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.8\columnwidth}
	\import{chap_MachineLearning/}{backpro_2.pdf_tex}
	\caption{The back propagation algorithm}
	\label{bp}
\end{figure}

\subsubsection{Gradient with respect to weights of output layer}
As depicted in Fig.\ref{bp}, the gradient of global loss $E$ with respect to weight $w_{jk}^o$ of output layer can be expressed by the chain rule
\begin{align}
\frac{\partial E}{\partial w^{o}_{jk}}=\frac{\partial E}{\partial o^{k}} \cdot \frac{\partial o^{k}}{\partial s^{o}_{k}} \cdot \frac{\partial s^{o}_{k}}{\partial w^{o}_{jk}}
\end{align}
where $s_k^o$ is the summed input of the neuron $k$ expressed as $s_k^o=\sum_{j=1}^{numh} h_j^{n} w_{jk}^o$ and $o_k=f_s(s_k^o)$ is the output of the neuron $k$ in output layer.
According to the expression of $s_k^o$, its derivative with respect to weight can be computed as
\begin{align}
\frac{\partial s^{o}_{k}}{\partial w^{o}_{jk}}=h_j^{n}.
\end{align}
Replace the first two terms of the right hand side fo eq.7.4 with 
\begin{align}
\delta_k^o=\frac{\partial E}{\partial s^{o}_{k}}=\frac{\partial E}{\partial o_{k}} \cdot \frac{\partial o_{k}}{\partial s^{o}_{k}},
\end{align}
the gradient of global loss in eq.7.4 can be represented as
\begin{align}
\frac{\partial E}{\partial w^{o}_{jk}}=\delta^o_k h_j^{n}.
\end{align}
\subsubsection{Gradient with respect to weights of hidden layer}
To compute the gradient of loss $E$ with respect to weight $w_{ij}^{n}$ as shown in Fig.\ref{bp}, the contributions of hidden neuron $h_j^n$ to all of the output neurons have to be accounted for in the chain rule
\begin{align}
\frac{\partial E}{\partial w^{n}_{ij}}= \left( \sum_{k=1}^{numo} \frac{\partial E}{\partial s^{o}_{k}} \cdot \frac{\partial s^{o}_{k}}{\partial h^{n}_{j}} \cdot \frac{\partial h^{n}_{j}}{\partial s^{n}_{j}}\right)  \cdot \frac{\partial s^{n}_{j}}{\partial w^{n}_{ij}}
\end{align}
where $numo$ is the number of neuron in the output layer, $s_j^n$ is the summed input of neuron $j$ in the $n$-th hidden layer, $h_j^n$ is the output of neuron $j$ and $w_{ij}^n$ is the weight of the connection between neuron $i$ and neuron $j$. Substituting eq.7.6 into eq.7.8 and simplifying the expression, it will lead to
\begin{align}
\frac{\partial E}{\partial w^{n}_{ij}}&= \left( \sum_{k=1}^{numo} \delta^o_k \cdot w_{jk}^o \right) \cdot \frac{\partial h^{n}_{j}}{\partial s^{n}_{j}}  \cdot h_i^{n-1}\\
&=\delta_j^n \cdot h_i^{n-1}
\end{align}
where $h_i^{n-1}$ is the output of neuron $i$ in the $(n-1)$-the hidden layer.

\subsubsection{Training algorithms}
To solve this optimization problem for neural network training, a proper optimizer has to be chosen to update the weights. Stochastic gradient descent (SGD), also known as incremental gradient descent, is an iterative method that can be used to get the minimized performance function and network weights. In SGD, the netwrok weights are updated by:
\begin{align}
w^{t+1} = w^{t}- \eta \cdot \frac{\partial E(\boldsymbol{W})}{\partial w^{t}}
\end{align}
where $t$ is the iteration number, $\eta$ is the learning rate. SGD has a simple formulation. However, it is difficult for the SGD algorithm to select the most appropriate learning rate, which will let the performance function converge to a local optimal resulting in a significant error in the application.

The most common choice of the training algorithm for the FNN is the Levenberg-Marquardt algorithm, which has the second-order training speed without having to compute the Hessian matrix. The Levenberg-Marquardt algorithm stems from the quasi-Newton method that starts from an expansion of the gradient of objective function:
\begin{align}
{\frac{\partial E}{\partial w_i^{n+1}}} ={\frac{\partial E}{\partial w_i^{n}}} + {\frac{\partial^2 E}{\partial (w_i^{n})^2}} \Delta w_i^n + O(\left\| \Delta w_i^n \right\|^2 )
\end{align}
where the second order derivatives contribute to the Hessian matrix
\begin{align}
H_{ij}=\frac{\partial^2 E}{\partial w_i^{n} \partial w_j^{n}}.
\end{align}
Since the large memory of $O(n^2)$ is required to compute and store the Hessian matrix and its inverse for the high dimensional loss function, the Hessian matrix is approximated, in the Levenberg-Marquardt algorithm, as
\begin{align}
\boldsymbol H=\boldsymbol J^T \boldsymbol J,
\end{align}
where $\boldsymbol J$ is the the Jacobian matrix that contains first derivatives of network errors $e$ with respect to the weights
\begin{align}
J_{ij} = \frac{\partial e_i}{\partial w_j^{n}}.
\end{align}
The Jacobian matrix can be obtained directly from the back propagation process directly, which is much cheaper than computing the Hessian matrix. In addition, the gradient of the loss function thus can be computed as
\begin{align}
\frac{\partial E}{\partial w_j^{n}} = \sum_{i=1}^{n} e_i \frac{\partial e_i}{\partial w_j^{n}},
\end{align}
or in matrix notation
\begin{align}
\nabla E = \boldsymbol J^T \cdot \boldsymbol e.
\end{align}
Finally, the weight will be updated as
\begin{align}
\boldsymbol w^{n+1} =\boldsymbol w^{n}- (\boldsymbol J^T \boldsymbol J +\mu \boldsymbol{I})^{-1} \boldsymbol J^T \cdot \boldsymbol e,
\end{align}
where the vector $\boldsymbol w^{n+1}$ contains the weights in the next iteration, $\mu$ is a parameter to adaptively control the speed of convergence. When $\mu$ is is zero, it reproduces the quasi-Newton method, which is faster and more accurate near an error minimum. When $\mu$ is large, it becomes the gradient descent algorithm.

(levenburg)https://de.mathworks.com/help/deeplearning/ref/trainlm.html

\subsection{Data generation for the FNN based hyper-elasticity}
In this section, the objective is to train the FNN to learn a hyper-elastic behaviour and then test it in the finite element analysis. The first task is to collect the data for hyper-elasticity. Instead of using the experimental data, the training data is generated by the analytical model in this part, which allows us to test the performance of the proposed FNN based model by comparing its simulation results with that by analytical model. As an example for hyper-elasticity, the neo-Hookean model is applied to generate the data and thus as the target to learn
\begin{align}
\boldsymbol \sigma = \frac{1}{2}\frac{\lambda}{J}(J^2 - 1) \boldsymbol{I} + \frac{\mu}{J}(\boldsymbol{b} - \boldsymbol{I})
\end{align}
where the Cauchy stress $\sigma$ and the left Cauchy Green tensor $\boldsymbol{b}$ are symmetric tensors. For the 2D problem, the inputs of the model can be chosen as $(J,b_{11}, b_{22}, b_{12})$, whereas the outputs are chosen as the stress components $(\sigma_{11}, \sigma_{22}, \sigma_{12})$. According to the input and the output, the architecture of the FNN can be determined as $4-n-3$ for instance, where one hidden layer with $n$ neurons is applied for this hyper-elastic law. Since the strain and stress have a one-to-one mapping in the design space of elasticity, the input data is generated by taking equally spaced points within the given range of each input.

Before training the FNN, the generated data is usually scaled to a specific range, such $(-1,1)$. Then the network will be trained using proper optimizer until the stop criteria is reached. At this point, the weights $\boldsymbol{W}$ and basis $\boldsymbol{b}$ will be saved as the model parameters. The FNN based material model is thus expressed as
\begin{align}
\boldsymbol\sigma^{NN}&=FNN(\boldsymbol b, J, \boldsymbol{W}, \boldsymbol B)\\
&=\boldsymbol{W} \boldsymbol b +\boldsymbol B
\end{align}
\subsection{The residual and tangent}
The machine learning based plasticity model can be used as the classical constitutive model in the finite element analysis. The residual for the static problem of a Newton solution process is now given by:
\begin{align}
\boldsymbol{R} (\boldsymbol{u})=\boldsymbol{f}-\int_\Omega \boldsymbol{B}^T \boldsymbol{\sigma}^{NN} d\Omega, \\
\boldsymbol{f}=\int_\Omega N_a \rho \boldsymbol{b} da- \int_{\partial\Omega} N_a \boldsymbol{t} da,
\end{align}
In which $\boldsymbol{\sigma}^{NN}$ is the stress computed from the machine learning based model. Due to the non-linearity, the iterative solution scheme is required to solve the displacement by the Newton's method. The stiffness is computed by taking the derivative of radium in terms of displacement
\begin{align}
\boldsymbol{K}_T = \frac{\partial \boldsymbol{R}(\boldsymbol{u})}{\partial \boldsymbol u}
\end{align}
Since the The residual vector and the tangent matrix for the Newton Rapson scheme are derived by the symbolic tool AceGen.

The displacement field can be computed as
\begin{align}
\boldsymbol{K}_T \Delta \boldsymbol{u}=  \boldsymbol{R}
\end{align}

\subsection{Testing the FNN based hyper-elasticity in FEM}
The first example is the uniaxial compression test of a plate in 2D. As shown in Fig.\ref{bargeo}, the pressure is imposed on the top surface of the bar, the other end of the plate is fixed in vertical direction. The material parameters for the neo-Hookean model used in the training data are set as $E=700,\nu=0.499$. The distributed load is given as $ q_0=-20$. The training data consist of 100 loading paths with 100 points on each. The FNN with 1 input layer, 1 hidden layer with 20 neurons and one output layer is used. The Levenberg-Marquardt algorithm is applied as the training optimizer. After 1000 training iterations, the mean squared error is decreased to $1e^{-8}$.

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.3\columnwidth}
	\import{chap_MachineLearning/}{bargeo.pdf_tex}
	\caption{Compression of plate}
	\label{bargeo}
\end{figure}

To test the FNN based constitutive model, the simulation results of the plate by use of the FNN model is compared with the simulation by the neo-Hooken model. It can be see from Fig.\ref{barneofnn} that the displacement in compression direction in both tests are very close, which validates the effectiveness of the FNN model. 

\begin{figure}[htb]
	\centering
	\subfigure[Neo-Hookean model]{\label{test1dplas}\includegraphics[width=60mm]{chap_MachineLearning/bar_neo.jpg}}
	\qquad
	\subfigure[With FNN based model]{\label{test1dplas}\includegraphics[width=60mm]{chap_MachineLearning/bar_neofnn.jpg}}
	\caption{Compression of a bar.}
	\label{barneofnn}
\end{figure}

To validate the above FNN based material model further, the second benchmark test with a cook's membrane problem is conducted in this part, where the left hand side of the membrane is fixed and the vertical force boundary condition is imposed on the right hand side as depicted in Fig.\ref{cookgeo}.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.4\columnwidth}
	\import{chap_MachineLearning/}{cookgeo.pdf_tex}
	\caption{cook's membrane problem}
	\label{cookgeo}
\end{figure}

The cook's membrane problem is simulated by use of the FNN model and the neo-Hookean model as well. As shown in Fig. \ref{cookneofnn}, the vertical displacement in both tests are very close to each other, which verifies the effectiveness of the trained FNN model.

\begin{figure}[!htb]
	\centering
	\subfigure[Neo-Hookean model]{\label{test1dplas}\includegraphics[width=70mm]{chap_MachineLearning/cook_neo.jpg}}
	\qquad
	\subfigure[With FNN based model]{\label{test1dplas}\includegraphics[width=70mm]{chap_MachineLearning/cook_neofnn.jpg}}
	\caption{Cook's membrane problem}
	\label{cookneofnn}
\end{figure}

To this end, it proves that the FNN works well for the nonlinear elastic behaviour as shown in the above results. The elastic deformation is a history independent process, which means its stress is only depend on its current kinematic variables. Hence, the feed forward neural network is enough to capture the behaviour. However, for a plastic behaviour, the response of the deformed material depends not only the current deformation but also on its deformation history. Since the FNN does not have any ability to record the loading history, it can not be used to learn the plasticity directly.

\section{Data collection strategy for plasticity}
(read the paper by Resse about plasticity in principle space)
Since the plastic deformation is path dependent, the data collection for plasticity will be quite different from that for elasticity. In this section, the data collection approach for von Mises plasticity will be introduced. 

For the von Mises elsto-plasticity, the material behaviour is distinguished by von Mises yield surface as shown in Fig.\ref{fig:yieldsurf} for the 2D case. Within the yield surface, the material behaves as elastic, where there is a one-to-one mapping relationship between the strain and stress. The material will behave as plastic when the current stress state is located outside this yield surface. Additionally, the response of the material will depend not only on the current strain but also on its loading history, such as the accumulated plastic strain. To learn the elato-plastic behaviour by the artificial neural network, the yield surface as well as the response in- and outside have to be captured. 

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.75\columnwidth}
	\import{chap_MachineLearning/}{von_mises_yieldsurf.pdf_tex}
	\caption{von Mises yield loci in 2D}
	\label{fig:yieldsurf}
\end{figure}
	
In Fig.\ref{fig:yieldsurf}, the yield surface is plotted in the principle space, where each point on the yield surface can be reproduced by some simple stress state in the general space, such as the tension, compression and the shear as depicted in Fig.\ref{fig:ele4}. However each stress state can be transformed to another state according to the Mohr's circle, where each point on the yield surface in principle space refers to multiple stress states in the general space. Thus unlimited choices can be made to represent the yield surface by stress data in general space, which complicates the data generation whether from experiments or simulations.\\

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.8\textwidth]{chap_MachineLearning/ele4.pdf}
	\caption{Stress state in general space (\textcolor{red}{???} plot other state)}
	\label{fig:ele4}
\end{figure}

Taking into account the accuracy requirement in neural network training, it is very important to have a concise and complete training data set, which contains enough information about the material behaviour but without too much repetition. Since all of the stress states on the yield surface on Fig.\ref{fig:yieldsurf} in the principle space can be can be transformed into the general space and vice versa, the data generation approach within the principle space is proposed for plasticity. In this way, only the principle stresses are enough to represent the yield surface. At the same time the isotropic plasticity can be formulated in the principle space, see [cite Resse's paper], thus the neural network based plasticity model will be formulated in the principle space accordingly, which will be consistent with the training process. Additionally, the formulation in principle space reduces the dimension of the input and output of neural networks.

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.75\columnwidth}
	\import{chap_MachineLearning/}{von_mises_yieldsurf3D.pdf_tex}
	\caption{von Mises yield loci in 3D}
	\label{fig:yieldsurf3D}
\end{figure}


\subsection{Small strain plasticity in principle space}
In this section, the formulation of small strain von Mises plasticity in principle space will be introduced. The small strain in continuum mechanics is computed as the symmetric part of the displacement gradient:
\begin{align}
	\boldsymbol\varepsilon=\frac{1}{2}(\boldsymbol{H}+\boldsymbol{H}^T)
\end{align}
where $\boldsymbol{H}$ is the displacement gradient with $\boldsymbol{H}=\boldsymbol{F}-\boldsymbol{1}$. By use of the spectral decomposition, the strain tensor can be formulated in the principle space:
\begin{align}
	\boldsymbol\varepsilon =\boldsymbol Q \cdot \boldsymbol\Lambda \cdot \boldsymbol Q^T.
\end{align}
where $\boldsymbol\Lambda$ is the principle strain after transforming into the principle space with the rotation matrix $\boldsymbol Q$. The multiplicative split of the deformation gradient in plasticity leads to the additively decomposition of the total small strain into elastic part and plastic part.
\begin{align}
	\boldsymbol\Lambda =\boldsymbol\Lambda^e +\boldsymbol\Lambda^p
\end{align}
The trial principle Cauchy stress is determined by a linear elastic law:
\begin{align}
	\boldsymbol \Sigma^{tr}=\lambda tr(\boldsymbol\Lambda^e) \cdot \boldsymbol{1}+2\mu \boldsymbol\Lambda^e,
\end{align}
where $\lambda$ is the bulk modulus and $\mu$ is the shear modulus. By assuming the von Mises yield criteria and the swift isotropic hardening law, the yield function is written as:
\begin{align}
	f=\sqrt{\frac{3}{2} \Vert\boldsymbol{s} \Vert} - (y_0+a\gamma^{0.028})
\end{align}
where $\boldsymbol{s}$ is the trial deviatoric stress with $\boldsymbol{s} = \boldsymbol\Sigma^{tr} - \frac{1}{3} tr\boldsymbol\Sigma^{tr} \cdot \boldsymbol{1}  $, $y_0$ is the initial yield stress, $\gamma$ is the accumulated equivalent plastic strain and $a$ is a parameter. By use of the associated plastic flow rule, the evolution of the principle plastic strain is formulated as:
\begin{align}
	\dot{\boldsymbol\Lambda}^p=\dot{\gamma}\frac{\partial f}{\partial \boldsymbol{s}}
\end{align}
where $\gamma$ is the plastic multiplier. By applying the return mapping algorithm, the increment of plastic multiplier and the elastic strain will be calculated by solving the yield equation and the evolution equation. The principle Cauchy stress can thus be updated by the linear elastic law. Then the Cauchy stress is computed by transforming the principle Cauchy stress into the general space
\begin{align}
	\boldsymbol\sigma =\boldsymbol Q \cdot \boldsymbol \Sigma \cdot \boldsymbol Q^T.
\end{align}
Based on the above formulation in principle space, the principle strain  $\boldsymbol \Lambda$ and principle stress $\boldsymbol \Sigma$ will be served as the input and output of the machine learning based plasticity model respectively.

\subsection{Concept of sequence for plasticity}
Since the plastic flow depends on not only the current total strain but also the accumulated plastic strain (loading history), the plastic deformation is a history dependent process. In other words, the strain and stress data sets at one integration point have strict order along the loading path, which can be written as two set of time series data or two corresponding sequences
\begin{align}
\lbrace \boldsymbol\varepsilon^1, \boldsymbol\varepsilon^2, \boldsymbol\varepsilon^3, ... \boldsymbol\varepsilon^t, ... \rbrace \Leftrightarrow \lbrace \boldsymbol\sigma^1, \boldsymbol\sigma^2, \boldsymbol\sigma^3, ... \boldsymbol\sigma^t, ... \rbrace.
\end{align}
Thus the basic data unit for plasticity model is not a strain-stress tensor pair but a strain-stress sequence pair. It can be noticed that multiple strain-stress sequences can be generated for one loading path with different loading increment. For a 1D loading case, the time series data of strain and stress for the plasticity model is shown in Fig.\ref{series1d}.\\ 

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.5\columnwidth}
	\import{chap_MachineLearning/}{sequence1d.pdf_tex}
	\caption{predict coefficient by FNN}
	\label{series1d}
\end{figure}

As a plasticity model, the stress sequence will be predicted for given strain sequences from any loading paths. Hence, to represent a plasticity model by sequence data, we have to collect the strain-stress sequence data along different loading paths under different loading cases as shown in Fig.\ref{fig:yieldsurf}.

\subsection{Data generation}
As a benefit of the formulation in principle space, the principle strain and principle stress data can be collected from the simple loading cases including tension and compression, which brings the convenience for data collection from the experiments and simulations. In this part, the data generation approach from simulations will be introduced.

To collect the strain-stress sequences from simulation, single finite element is applied by imposing specific motion on the nodes. As shown in Fig.\ref{ele4}, Q1 element is applied for the 2D case, where both the tension and compression loading state can be obtained by moving the node $A, B$ and $C$ where as node $O$ is fixed. With the displacements $u_x$ and $u_y$, the element will undergo specific deformations. Since the deformation of the element is only limited to tension or compression, the amount of the deformation can be characterized by the displacement $(u_x, u_y)$ of the node $A$.

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.4\columnwidth}
	\import{chap_MachineLearning/}{ele4-biaxialtension.pdf_tex}
	\caption{Biaxial tension}
	\label{ele4}
\end{figure}
 To generate the sequence data from loading path, the loading path for this element has to be defined firstly. According to the tension and compression of the element depicted in Fig.\ref{ele4}, the loading path can be determined according to the displacement of node $A$. As shown in Fig.\ref{path-circle}, the loading path $OP$ indicates the trajectory of the node $A$, where the displacement of node $A$ increases from zero to the maximum value at point $P$ on the circle proportionally. By setting the position of the point $P$ on a circle with the angle $\phi$, the loading paths can be determined. The radius of the circle determines the amount of loading. To include the information of the whole yield surface, the enough loading paths around the circle have to be generated. Along one loading path, multiple strain-stress sequences can be generated with different loading increments. \\
  
\begin{figure}[htb]
	\centering
	\def\svgwidth{0.4\columnwidth}
	\import{chap_MachineLearning/}{circle.pdf_tex}
	\caption{Biaxial tension (plot the circle of loading paths)}
	\label{path-circle}
\end{figure}

For the 3D case, the cubic element is applied, as shown in Fig.\ref{ele8}, where the amount of deformation for tension or compression can be characterized by the displacement $(u_x, u_y, u_z)$ of the node $A$. \\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.5\columnwidth}
	\import{chap_MachineLearning/}{ele8-biaxialtension.pdf_tex}
	\caption{Biaxial tension}
	\label{ele8}
\end{figure}
The loading path for 3D case is generated in the spherical coordinate system as shown in Fig.\ref{path-sphere}. The displacement of node $A$ increases along the path $OP$ to a maximum value on the sphere. The loading path $OP$ is distinguished by the angles $\phi$ and $\theta$. To include the information of the 3D yield surface, enough loading paths have to be generated with different angles.\\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.5\columnwidth}
	\import{chap_MachineLearning/}{sphere.pdf_tex}
	\caption{Biaxial tension (plot the circle of loading paths)}
	\label{path-sphere}
\end{figure}

After the data generation, the machine learning technology is applied to develop the data-driven material model. In this work, the neural networks is applied for the data-driven material modelling. To predict the path dependent material behaviour in plasticity by neural networks, one solution is to attach the history variable as the additional input of feed forward network. In literature, the stress and strain in the last step are applied as the history information together with the current strain in the input. However, the previous strain and strain is not enough to distinguish the load history in the real application. In addition, the previous stress, which is predicted by the neural network with error included, will introduce extra error into the system in an accumulate way. In this work, a different history variable is selected as the additional input of feed forward neural networks together with the Proper Orthogonal Decomposition (POD), which will be introduced in the following section. Another solution for the time series problem is to apply the recurrent neural network that has the memory function because of its different internal architecture, which will be introduced in the following section 7.5.

\section{Recurrent Neural Network (RNN) based constitutive model}
The recurrent neural networks has been applied in many fields to solve the sequential problem, such as the recognition of speech and prediction of time-varying patterns in dynamic system. Since the recurrent neural networks applies their internal state (memory) to deal with the input sequences, the history dependent variables can be predicted without including the history information in the inputs. According to the analysis in section *, the strain-stress data along the loading paths in plasticity model are time sequences. Based on the above feature, the RNN is applied to model the elasto-plastic behaviour in this work.

\subsection{Network architecture}
As shown in Fig.\ref{RNN1}, the RNN is composed of an input layer, a hidden layer with the Long Short Term Memory (LSTM) neurons and an output layer. As same as the feed forward neural networks, the hidden layer of the recurrent neural networks is fully connected with the input layer and the output layer respectively. However, the hidden layer of recurrent neural networks contains the specially design neurons, the Long Short Term Memory (LSTM) neurons, where the feed back information from the last output of the neurons will be included in the current input.\\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.5\columnwidth}
	\import{chap_MachineLearning/}{RNN1.pdf_tex}
	\caption{The recurrent neural networks (RNN)}
	\label{RNN1}
\end{figure}

To get a better understanding, the data flow of the LSTM neuron is unfolded with the time steps as shown in Fig.\ref{RNN2}. The unfolded LSTM neuron can be seen as a copied chain-like networks along the time series, where each LSTM neuron will receive the history information the previous one and then pass the information (cell state $\boldsymbol{c}_t$ and hidden state $\boldsymbol{h}_t$) to its successor within each prediction step. At the same time, the network predicts an output $\boldsymbol{y}_t$ based on the current input $\boldsymbol{x}_t$ and the history information at each time step. Thus, the input and the output of the LSTM neuron can be seen as the sequence data, which allows the recurrent neural network to deal with the sequences. If the strain sequence is applied as the input and the stress sequence is applied as the output, the history dependent plasticity behaviour can be learned by the LSTM neuron within the recurrent neural networks, which is the idea of this study.\\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.8\columnwidth}
	\import{chap_MachineLearning/}{RNN2.pdf_tex}
	\caption{The undolded recurrent neural networks }
	\label{RNN2}
\end{figure}

\subsection{The RNN based plasticity model}
To develop the neural networks based plasticity model, the formulations of the recurrent neural networks as well as the LSTM neuron is introduced in the following:
\subsubsection{Input layer}
Similar to the feed forward neural networks based model, the principle strain is employed as the input of the RNN based plasticity model. Thus it is required to transform the total strain into the principle space by the spectral decomposition
\begin{align}
\boldsymbol\varepsilon^t =\boldsymbol{Q} \boldsymbol\Lambda \boldsymbol{Q}^T
\end{align}
where $\boldsymbol\varepsilon$ is the total strain matrix, $\boldsymbol{Q}$ is the square matrix whose columns are the eigenvectors of $\boldsymbol\varepsilon$, $\boldsymbol\Lambda$ is the diagonal matrix whose diagonal elements are the eigenvalues of $\boldsymbol\varepsilon$.

Before feeding into the input layer, the principle strain has to be scaled into a specific range, which allows the activation functions to work within their sensitive regions. The strain component $\varepsilon_{i,t}$ at time $t$ is scaled as:
\begin{align}
\varepsilon^s_{i,t}=v_{min}+(v_{max}-v_{min})\frac{\varepsilon_{i,t}-\varepsilon_{min}}{\varepsilon_{max}-\varepsilon_{min}}, \;\; i=1,2,3.
\end{align}
where $\varepsilon^s_{i,t}$ is the scaled strain, $\varepsilon_{max}$ and $\varepsilon_{min}$ are the maximum and minimum value of the input strain, $v_{max}$ and $v_{min}$ are the scaling limits. The range of the input data and the scaling data will be identical for both training and testing of the neural networks. Thus the input $\boldsymbol{x}_t$ of the networks is a vector written as
\begin{align}
\boldsymbol{x}_t=\left\lbrace \boldsymbol\varepsilon^s_{1,t}, \boldsymbol\varepsilon^s_{2,t}, \boldsymbol\varepsilon^s_{3,t} \right\rbrace . \;\;\; [Ni \times 1]
\end{align}
Since the neurons in input layer are fully connected with the hidden layer, the input $\boldsymbol{x}_t$ will be feed into the hidden layer by multiplying the weighs. 

\subsubsection{Hidden layer}
As the cores of the recurrent neural networks, the LSTM neurons play very important role in hidden layer of the recurrent neural networks. The LSTM has the memory on its history information and thus can learn long-term dependencies between time steps of sequence data. The LSTM neuron is composed by four gates: the forget gate $f$, the input gate $(g,i)$ and the output gate $o$, as shown in Fig.\ref{LSTM}. The forget gate controls the length of the network memory. The history information is contained by the cell state and the hidden state. The input ${x}_t$ and the state variables $(c_{t-1}, h_{t-1})$ are feed into the neuron from the left hand side, then the data flows from the left hand side to the right hand side of the LSTM neuron by passing through all of the gates. Finally, the neuron will export an output $y_t$ and the state variable $(c_t,h_t)$.\\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.8\columnwidth}
	\import{chap_MachineLearning/}{LSTM.pdf_tex}
	\caption{The architecture of the LSTM neuron}
	\label{LSTM}
\end{figure}

In the hidden layer of the RNN, there are multiple LSTM neurons fully connected with the input layer. Thus the input, output and state variables of the LSTM neurons in hidden layer will be stored as vectors. The gate vectors $\boldsymbol{f}_t, \; \boldsymbol{g}_t, \; \boldsymbol{i}_t$  and $\boldsymbol{o}_t$ of the hidden layer are obtained from the input vector $\boldsymbol{x}_t$ and the hidden state vector $\boldsymbol{h}_{t-1}$, which are formulated as
\begin{align}
\boldsymbol{f}_t=sigmoid(\boldsymbol{W}_f \cdot \boldsymbol{x}_t + \boldsymbol{R}_f \cdot \boldsymbol{h}_{t-1}+\boldsymbol{b}_f)\\
\boldsymbol{g}_t=tanh(\boldsymbol{W}_g \cdot \boldsymbol{x}_t + \boldsymbol{R}_g \cdot \boldsymbol{h}_{t-1}+\boldsymbol{b}_g)\\
\boldsymbol{i}_t=sigmoid(\boldsymbol{W}_i \cdot \boldsymbol{x}_t + \boldsymbol{R}_i \cdot \boldsymbol{h}_{t-1}+\boldsymbol{b}_i)\\
\boldsymbol{o}_t=sigmoid(\boldsymbol{W}_o \cdot \boldsymbol{x}_t + \boldsymbol{R}_o \cdot \boldsymbol{h}_{t-1}+\boldsymbol{b}_o)
\end{align}
where $\boldsymbol{W}_f$, $\boldsymbol{W}_g$, $\boldsymbol{W}_i$ and $\boldsymbol{W}_o$ are the input weights corresponding to the four gates; $\boldsymbol{R}_f$, $\boldsymbol{R}_g$, $\boldsymbol{R}_i$ and $\boldsymbol{R}_o$ are the recurrent weights for the four gates; $\boldsymbol{b}_f$, $\boldsymbol{b}_g$, $\boldsymbol{b}_i$ and $\boldsymbol{b}_o$ are the biases; $tanh()$ denotes the hyperbolic tangent activation function
\begin{align}
tanh(x)=\frac{e^{2x}-1}{e^{2x}+1};
\end{align}
$sigmoid()$ denotes the sigmoid activation function:
\begin{align}
sigmoid(x)=\frac{1}{1+e^{-a(x-c)}},
\end{align}
where $a$ and $c$ are the function parameters. The value of the parameters are assigned as: $a=1, c=0$ in this work. In the implementation, the weight matrices are stored as
\begin{align}
\boldsymbol{WI}=
\left[ \begin{array}{r}
W_i\\W_f\\W_g\\W_o\\
\end{array}\right]_{[4Nh \times Ni]}, \;\;\;
\boldsymbol{WR}=
\left[ \begin{array}{r}
R_i\\R_f\\R_g\\R_o\\
\end{array}\right]_{[4Nh \times Nh]}, \;\;\;
\boldsymbol{BI}=
\left[ \begin{array}{r}
b_i\\b_f\\b_g\\b_o\\
\end{array}\right]_{[4Nh \times 1]}.
\end{align}
where $Ni$ is the number of input, $Nh$ is the number of hidden neuron in the LSTM layer.

After the gate values are determined, the cell state $\boldsymbol{c}_t$ and the hidden state $\boldsymbol{h}_t$ for the next step will be updated as:
\begin{align}
\boldsymbol{c}_t=\boldsymbol{f}_t \odot \boldsymbol{c}_{t-1} + \boldsymbol{i}_t \odot \boldsymbol{g}_{t}\\
\boldsymbol{h}_t=\boldsymbol{o}_t \odot tanh(\boldsymbol{c}_t)
\end{align}
where the symbol $\odot$ denotes the element weise multiplication of two vectors. The output of the hidden layer $\boldsymbol{y}_t$ is identical with the hidden state $\boldsymbol{h}_t$.

\subsubsection{Output layer}
As shown in Fig.\ref{RNN1}, a fully connected regression layer is attached behind the hidden layer in the RNN. The output of the RNN can be computed from the output of the hidden layer as
\begin{align}
\boldsymbol \sigma^s_t=\boldsymbol{W}_{out,[No \times Nh]} \cdot \boldsymbol{h}_t  +\boldsymbol{b}_{out,[No \times 1]}
\end{align}
where $\boldsymbol{W}_{out}$ and $\boldsymbol{b}_{out}$ are the weight and bias of the output layer. Since the stress has been scaled to the range $(q_{min},q_{max})$ during training, the output of the RNN $\boldsymbol \sigma^s_t$ is the scaled value of stress. The real value of stress can be descaled as:
\begin{align}
\sigma_{i,t}=\sigma_{min}+(\sigma_{max}-\sigma_{min})\frac{ \sigma^s_{i,t}-q_{min}}{q_{max}-q_{min}}
\end{align}
where $\sigma_{max}$ and $\sigma_{min}$ are the maximum and minimum value of the real stress.

The principle stresses obtained from neural networks have to be transformed into the principle space for the finite element application. By using the same transformation matrix $\boldsymbol{Q}$ in decomposition of strain, the Cauchy stress can be compute as
\begin{align}
\boldsymbol\sigma_t =\boldsymbol{Q}\boldsymbol\Sigma\boldsymbol{Q}^T
\end{align}
where lumped matrix $\boldsymbol \Sigma$ contains the principle stress components.

\subsection{Residual and tangent matrix}
To apply the above RNN based plasticity model in the finite element analysis, the residual vector and tangent matrix is derived in this section. The RNN based plasticity model defines an incremental constitutive function in the following format
\begin{align}
\boldsymbol \sigma_t=\hat{\boldsymbol \sigma} (\boldsymbol \varepsilon_t \mid \boldsymbol{h}_{t-1},\boldsymbol{c}_{t-1}, \boldsymbol{W}).
\end{align}
where $\boldsymbol{W}$ denotes all of the weights of neural networks. By use of the nodal-wise assembly of the discretized equation of motion, the residual of each integration point has the form
\begin{align}
\boldsymbol R_p = \sum_{i=1}^{n} \boldsymbol{B}_{ip} \boldsymbol{\sigma}_{NNp} v_p
\end{align}
where $\boldsymbol{B}_{ip}$ is the derivative of shape function $N$, $v_p$ is the current volume of the element. The tangent matrix is formulated as
\begin{align}
\boldsymbol K_p = \frac{\partial \boldsymbol R_p}{\partial \boldsymbol u}
\end{align}
The automatic differentiation tool AceGen is applied to derive the tangent.

\subsection{Training the RNN}
According to the above description, the input and output of recurrent neural networks are sequence data. Thus, the strain-stress sequences generated in section 7.3 will be served as the training data. To train the recurrent neural networks, the back propagation algorithm will be employed as well to compute the gradients. The mean squared error is applied to evaluate the difference between the neural network prediction and the target value during the training progress. The Adam algorithm is applied as the training algorithm for the recurrent neural networks, which will be introduced in following.

\subsubsection{Training algorithm}
Adam, fully named as adaptive momentum estimation, is also a gradient based method, which seeks to improve network training by using different learning rates for different weights and the adaptive learning rates for each optimization step. The algorithm computes the moving averages of the gradients and its squared values
\begin{align}
m_i^n=\beta_1\cdot m_i^{n-1}+(1-\beta_1)\cdot {\frac{\partial E(\boldsymbol{w})}{\partial w_i^{n}}}\\
v_i^n=\beta_2\cdot v_i^{n-1}+(1-\beta_2)\cdot \left[ {\frac{\partial E(\boldsymbol{w})}{\partial w_i^{n}}}  \right]^2
\end{align}
where $m_i^n$ and $v_i^n$ are the estimates of the first moment (the mean) and the second moment (the uncentered variance) of the gradients respectively. $\beta_1$ and $\beta_2$ are the gradient decay factor and squared gradient decay factor respectively. The network weights are updated by the moving averages as:
\begin{align}
w_i^{n+1}=w_i^n-\alpha \frac{m_i^n}{\sqrt{v_i^n}+\epsilon}
\end{align}
where $\alpha$ is the learning rate, $\epsilon$ is a parameter which makes the denominator nozero. The common values of $\beta_1$, $\beta_2$ and $\epsilon$ are $0.9$, $0.999$ and $10^{-8}$ respectively.
link: https://de.mathworks.com/help/deeplearning/ref/trainingoptions.htmlbu59f0q-ExecutionEnvironment

\subsubsection{Adaptive learning rate schedule}
The learning rate $\alpha$ is an important argument of the Adam optimizer. The learning rate is initialized by a specific value by experimenting with different values. Instead of using constant learning rate during training,  the learning rate is gradually reduced as the training progresses, which allows the optimization converges to a the global minimum and cirmuvements the oscillation when the  error becomes very small. The learning rate reduction can be conducted by using pre-defined learning rate schedules. In this work, the Step decay schedule is applied where the learning rate is reduced by a factor of 0.2 every 2000 epochs.


\subsection{Testing of the RNN based plasticity model}
\subsubsection{Uniaxial tension and compression}
To test the performance of the RNN based elasto-plastic model, the uniaxial tension and compression test is conducted firstly. The plasticity model used in section 7.4.4 for uniaxial tension and compression test is applied as the learning target in this part. The training data composed of 11 sets of strain-stress sequences is generated according to the 1D plasticity model, where the strain increments increases linearly from 0.* to 0.*. The training data sets are plotted in Fig.\ref{train1dplas}.\\
\begin{figure}[!htb]
	\centering
	\includegraphics[width=0.6\textwidth]{chap_MachineLearning/train_1dplas.jpg}
	\caption{training data}
	\label{train1dplas}
\end{figure}
The RNN with an architecture of (1-10-1) is applied, where the input layer with 1 neuron is connected with the hidden layer composed of 10 LSTM neurons. A fully connected layer with 1 neuron is attached as the output layer. The input of the RNN is the total strain sequence and the output is the stress sequence. After *** epochs of training, the mean squared error is decreased to ** and the training progress is terminated.

The RNN based material model is tested by feeding a total strain sequence with a different data density from training data sets. The predicted stress and the analytical stress are plotted in Fig.\ref{test1dplas}. It can be observed that the predicted stress follows the target solution quite well.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{RNN1D.pdf_tex}
	\caption{Uniaxial tension and compression.}
	\label{test_1dplas_RNN}
\end{figure}


\subsubsection{Application to the FEM analysis}
The application of the RNN based elasto-plasticity model in finite element applications will be evaluated in this part. To prepare the training data, the strain-stress sequences are generated by the biaxial tension and compression test introduced in the section 7.3. The von Mises plasticity with a exponential isotropic hardening law is selected as the target plasticity model to learn, where the material parameters are set as Young's modulus $E=1$, Poison's ratio $\nu=0.33$, yield stress $\sigma_y=0.05$ and isotropic hardening parameter $H_{iso}=0.1$. There are 150 loading paths in Fig.\ref{path-circle} are employed and 5 strain-stress sequences are generated for each loading path with different strain increment.

The network architecture (2-20-2) is applied for the recurrent neural networks, where both the input layer and output layer contain 2 neurons, and a hidden layer with 20 LSTM neurons is fully connected in between. The principle total strain sequences are served as the inputs whereas the principle stress sequences are serves as the outputs. In the Adam training algorithm, the initial learning is set to be 0.01 and then drops with a factor of 0.8 every 2000 epochs. The training progress is terminated after 2000 epochs of training, when the mean squared error is decreased to $3 \times 10^{-4}$.

After the training, the weights and biases of the RNN are stored as the constant parameters for the RNN based plasticity model described equation (7.63). The tangent matrix and the residual vector of the finite element formulation are derived using the symbolic differentiation tool AceGen. 

Firstly, the 2D RNN based plasticity model is tested by the Cook's membrane problem introduced in Fig.\ref{cookgeo2D}. A constant distributed vertical load $q_0=0.03$ is loaded at the right end of the beam. The geometric domain of the structure is discretized by 40 elements with 189 nodes, where the quadratic finite element with 9 nodes is employed.

Fig.\ref{cook} shows the final deformation state of the membrane. It can be observed that the displacement in y direction computed by the RNN based plasticity model has a good agreement with that by the J2 plasticity mode.\\

\begin{figure}[!htb]
	\centering
	\subfigure[traing data]{\label{cookj2}\includegraphics[width=60mm]{chap_MachineLearning/RNN-cook.jpg}}
	\qquad \qquad \qquad
	\subfigure[testing]{\label{cookrnn}\includegraphics[width=60mm]{chap_MachineLearning/RNN-cookNN.jpg}}
	\caption{Training and testing the uniaxial tension/compression.}
	\label{cook}
\end{figure}

The load deflection curve of the upper node $(48, 60)$ is plotted in Fig. \ref{cookfu}, where the results by RNN model is compared with that by the J2 plasticity model. It can be observed that the \\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{RNN-cook.pdf_tex}
	\caption{Uniaxial tension and compression.}
	\label{RNNcook}
\end{figure}

\section{Feed forward neural network based elasto-plasticity}
In this section, the machine learning approach of combining the Proper Orthogonal Decomposition (POD) with the feed forward neural network is proposed to develop a data-driven plasticity model. Firstly, the Cauchy stress sequence is represented by the POD. Based on this, the machine learning based plasticity model is formulated with the POD representation of the stress, where the coefficients in the POD representation are predicted by the FNN. And of course the  training data generated in the last section will be transformed ba the POD. Finally, the developed plasticity model is validated within the finite element framework.
\subsection{POD}

\subsection{Represent the stress by POD}
(extent to 3D)\\
The Proper Orthogonal Decomposition (POD) has been used to characterize the vector field evolving with time in computational fluid mechanics. By use of the POD, the time series vector variables can be represented with a low number of modes, where the higher order modes can be neglected when the error is acceptable. Thus, by use of the POD, the problem will be decoupled into a combination of several different modes. As a time series data, the stress sequence can be written as the snapshot matrix
\begin{align}
\boldsymbol B=
\begin{bmatrix}
\boldsymbol \sigma^1 & \boldsymbol \sigma^2 & ... & \boldsymbol \sigma^t & ... 
\end{bmatrix}
=
\begin{bmatrix}
\sigma^1_x & \sigma^2_x & ... & \sigma^t_x & ...\\
\sigma^1_y & \sigma^2_y & ... & \sigma^t_y & ...
\end{bmatrix}, \,\, (t=1,...,M),
\end{align}
where $\boldsymbol{\sigma}^t$ is the principle stress vector with the components $(\sigma_x^t, \sigma_y^t, \sigma_z^t)$ and $M$ is the length of the sequence. The objective of POD is to represent the vector field at any time step by use of a linear combination of basis vectors and its coefficients. For instance, the principle stress at time $t$ will be represented as
\begin{align}
\boldsymbol \sigma^t_{POD} = 
\begin{bmatrix}
\bar{\sigma_x}\\
\bar{\sigma_y}
\end{bmatrix} 
+ \boldsymbol U_{2\times2} \boldsymbol \alpha^t_{2\times1}
\end{align}
where $\boldsymbol U$ is the basis matrix, $\boldsymbol \alpha^t$ is the coefficient matrix. $\bar{\sigma_x}$ and $\bar{\sigma_y}$ are the mean values of each row of snapshot matrix, which are computed as
\begin{align}
\bar{\sigma_x}=\frac{1}{M}\sum_{i=1}^M \sigma^i_x, \,\,\,\bar{\sigma_y}=\frac{1}{M}\sum_{i=1}^M \sigma^i_y.
\end{align}
To obtain the POD representation, the basis and its coefficients have to be determined. According to Newman (1996), the basis is the eigenvectors of the covariance matrix $\boldsymbol C$, which is calculated as
\begin{align}
\boldsymbol C=\boldsymbol B_{dev} \boldsymbol B_{dev}^T,
\end{align}
where $\boldsymbol B_{dev}$ is the deviatoric snapshot matrix
\begin{align}
\boldsymbol B_{dev}=\boldsymbol B - \boldsymbol B_{mean}
\end{align}
with 
\begin{align}
\boldsymbol B_{mean}=
\begin{bmatrix}
\bar{\sigma_x} & \bar{\sigma_x} & ... & \bar{\sigma_x} & ...\\
\bar{\sigma_y} & \bar{\sigma_y} & ... & \bar{\sigma_y} & ...
\end{bmatrix}.
\end{align}
In practice, the basis $\boldsymbol U$ is computed from the Singular Value Decomposition
 (SVD) of the deviatoric snapshot matrix:
\begin{align}
\boldsymbol B_{dev}=\boldsymbol U \boldsymbol S \boldsymbol V^T,
\end{align}
where $\boldsymbol U$ and $\boldsymbol V$ are the unitary matrix, $\boldsymbol S$ is the rectangular diagonal matrix with non-negative real numbers on the diagonal. Since the number of non-zero column in $\boldsymbol U$ is equal to the rank of $ \boldsymbol B_{dev}$, in the following, we just use the non-zero columns of $\boldsymbol U$. The coefficient $\boldsymbol \alpha^t$ can be obtained by projecting of the  snapshots on the basis
\begin{align}
\boldsymbol \alpha^t_{2\times M}=\boldsymbol U^T_{2\times2} \boldsymbol B^t_{dev}.
\end{align}

By use of POD, the stress sequence is decoupled into several independent coefficient sequences and the associated basis. Since the basses are independent of each other, the coefficient are independent as well. Thus the original strain-stress relationship in the plasticity model is decoupled into the relation between the strain and each independent coefficient, which can be written as
\begin{align}
\lbrace \boldsymbol\varepsilon^1, \boldsymbol\varepsilon^2, \boldsymbol\varepsilon^3, ... \boldsymbol\varepsilon^t, ... \rbrace \Leftrightarrow \lbrace \alpha^1_i, \alpha^2_i, \alpha^3_i, ... \alpha^t_i, ... \rbrace, (i=1,2,3),
\end{align}
where the coefficients $\alpha_1$, $\alpha_2$ and $\alpha_3$ are independent with each other.

\subsection{Neural network based plasticity model}
Based on the POD representation of the stress in the last section, the machine learning based plasticity model can be proposed
\begin{align}
\boldsymbol \sigma^t_{POD} = 
\begin{bmatrix}
\bar{\sigma_x}\\
\bar{\sigma_y}
\end{bmatrix} 
+ \boldsymbol U_{2\times2} \boldsymbol \alpha^t_{NN}
\end{align}
where the coefficient will be predicted by the feed forward neural networks as
\begin{align}
\alpha^t_i = FNN_i (\boldsymbol \varepsilon^t,\boldsymbol \varepsilon_{acc}^t, \boldsymbol W).
\end{align}
In the neural networks, the input is the principle strain and the accumulated absolute strain, the output is the coefficient. The principle strain is obtained by the spectral decomposition of the total strain.

Finally, the principle Cauchy stress $\boldsymbol \sigma^t_{POD}$ in eq.(7.42) will be transformed to the general space:
\begin{align}
\boldsymbol\sigma^t =\boldsymbol{Q}\boldsymbol \sigma^t_{POD}{Q}^T
\end{align}

The following section will introduce how to learn the pattern between the strain sequences and the coefficient sequences in Equation 7.41 by use of the neural networks.

\subsubsection{predict $\alpha$ by FNN}
In the prediction phase, the coefficient $\alpha$ corresponding to a given strain has to be predicted while the the basis $\boldsymbol U$ from the training data is retained. In this work, the feed forward neural networks is applied to predict the coefficient sequences, where the history variable have to be used as the additional input.

Since the coefficients in the POD representation are independent, we can predict the coefficients separately, i.e. each coefficient will be predict by their own neural networks, as shown in Fig.\ref{FNN}. Without the POD decomposition, single neural network will be applied to predict the stress, where the strain components will be the input and the stress components will be the outputs. With the POD decomposition, the stress  is replaced by the independent coefficients and the constant basis, which makes the original neural networks with multiple outputs become decoupled neural networks with only one output. Additionally, with only one output, it will be easer to train the neural networks.\\

\begin{figure}[htb]
	\centering
	\def\svgwidth{0.84\columnwidth}
	\import{chap_MachineLearning/}{FNN.pdf_tex}
	\caption{Coefficients predicted by FNN.}
	\label{FNN}
\end{figure}

After the POD, the strain-stress sequence is decoupled into the strain-coefficient sequence, where coefficient sequence is still a history dependent problem. To predict the coefficient sequence by neural networks, the history information have to be included in the input of the neural networks in some way that it can distinguish the loading history. 

The choice of the input and output for neural network is crucial for a successful approximation of constitutive model, especially the history variable for path dependent model. In this work, the accumulated absolute strain is applied in the input of FNN as the history variable. The accumulated absolute strain can be obtained by adding up all the absolute value of strain increments contentiously
\begin{align}
\boldsymbol \varepsilon_{acc}^t=
\begin{cases}
\boldsymbol \varepsilon_{acc}^{t-1} + \lvert \varepsilon^{t-1} - \lvert \varepsilon^{t-2} \rvert, & \text{if $t>2$},\\
0, & \text{otherwise}.
\end{cases}
\end{align}
The advantage of choosing the accumulated strain is that it can be obtained from the existing input data and does not need to prepare additional data. Thus the coefficient $\alpha^t_i$ at time $t$ will be predicted by the feed forward neural networks $FNN_i$ as
\begin{align}
\alpha^t_i = FNN_i (\boldsymbol \varepsilon^t,\boldsymbol \varepsilon_{acc}^t, \boldsymbol W)
\end{align}
where $i$ indicates the number of the coefficient, $\boldsymbol \varepsilon^t$ is the current strain, $\boldsymbol \varepsilon_{acc}^t$ is the accumulated absolute strain and $ \boldsymbol W$ is the weight matrix of neural networks. In the case of 3D plasticity model in principle space, the input and output data will be 
\begin{align}
\begin{bmatrix}
\varepsilon_x^t\\
\varepsilon_y^t\\
\varepsilon_{acc,x}^t\\
\varepsilon_{acc,y}^t
\end{bmatrix} 
\rightarrow 
\begin{bmatrix}
\alpha_x^t\\
\alpha_y^t
\end{bmatrix}
\end{align}
To train the above neural networks, the training data can be obtained by transforming the stress data in Section 2 with POD.

\subsection{Residual and tangent matrix}
To apply the above neural networks based plasticity model in the finite element analysis, the residual vector and tangent matrix has to be derived. The formulation of the machine learning based material model defines an incremental constitutive function in the following format:
\begin{align}
\boldsymbol \sigma_{NN}^t=\hat{\boldsymbol \sigma} (\boldsymbol \varepsilon_t \mid \boldsymbol{\varepsilon}_{acc}^t,\boldsymbol{W}).
\end{align}
where $\boldsymbol{\varepsilon}_{acc}^t$ is the history variable defined in equation (7.45), $\boldsymbol{W}$ is the weights of neural networks. 

By use of the nodal-wise assembly of the discretized equation of motion, the residual of each integration point has the form
\begin{align}
\boldsymbol R_p = \sum_{i=1}^{n} \boldsymbol{B}_{ip} \boldsymbol{\sigma}_{NNp} v_p
\end{align}
where $\boldsymbol{B}_{ip}$ is the derivative of shape function $N$, $v_p$ is the current volume of the element. The tangent matrix is formulated as
\begin{align}
\boldsymbol K_p = \frac{\partial \boldsymbol R_p}{\partial \boldsymbol u}
\end{align}
If the tangent matrix is derived manually, the back propagation process has be be applied, which will be very tricky in case that there is a large number of neurons and weights. To calculate the partial differentiation efficiently, the automatic differentiation tool AceGen is applied, which is based on the Mathematic symbolic computing in Mathematica, see Korelc and Wriggers book.

\subsection{Testing the FNN+POD model in FEM}
\subsubsection{Uniaxial tension and compression}
To test the performance of the POD-FNN based elasto-plastic model, the 1D uniaxial tension and compression test is conducted. The elasto-plasticity with the linear isotropic hardening is applied as the target model to learn. The material parameters of the plasticity model are set as: Young's modulus $E=700$, yield stress $\sigma_y=100$ and isotropic hardening parameter $H_{iso}=10$. To prepare the training data, 11 sets of strain-stress sequence data is generated based on the plasticity model with a strain increment increased linearly from $0.02$ to $0.03$. The stress sequences are then transformed into the coefficient sequence by the POD. 

The feed forward neural network with architecture of (2-20-20-1) is applied to predict the coefficient, where the input layer containing 2 neurons is connected with two hidden layers containing 20 neurons each. The output layer contains one neuron. The input of the neural network is the total strain sequences together with the accumulated absolute strain, and the output of the neural network is the coefficient sequences transformed from the stress sequence. The Bayesian regression is applied as the training algorithm. After 4000 epochs of training, the mean squared error is decreased to 0.0329 and the training progress is terminated.

The testing strain sequence is generated by setting the strain increment as 0.15 so that it is different from the training data. The stress computed from the neural network based plasticity model is compared with the the stress from the classical plasticity model, as shown in Fig.\ref{POD1D}. It can be seen that the predicted stress follows the exact solution quite well, which validates the effectiveness of the proposed machine learning approach for plasticity. \\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{POD1D.pdf_tex}
	\caption{Uniaxial tension and compression.}
	\label{POD1D}
\end{figure}

\subsubsection{Applications in 2D finite element analysis}
To evaluate the machine learning based elasto-plasticity further, the benchmark tests in 2D and 3D finite element applications will be presented in the following. To generate the training data, one Q1 finite element is applied with the loading condition of the biaxial tension and compression described in section 7.3.3. The von Mises plasticity with a exponential isotropic hardening law $\sigma_y = y_0+y_0(0.00002+\gamma)^{0.3}$ is set as the target model. The material parameters are set as Young's modulus $E=1$, Poison's ratio $\nu=0.33$, and the initial yield stress $y_0=0.05$. In the training data preparation, the strain-stress sequences under 150 loading paths are generated based on the description in Fig.\ref{path-circle}. Then the coefficient sequences corresponding to the stress sequences are obtained by POD.

Since there are two coefficients referring to the two principle stress components in the 2D case, two neural networks will be required to predict the coefficient. In this part, the same network architecture (4-20-20-1) is applied for the two feed forward neural networks, where the input layer containing 4 neurons is connected with two hidden layers containing 20 neurons each. The output layer contains always one neuron. The total strain sequences together with the accumulated absolute strain are applied as the input of the neural networks. The output of the neural network is the coefficient sequences transformed from the stress sequences. The Bayesian regression is applied as the training algorithm as well. After 2000 epochs of training for each neural networks, the mean squared errors are decreased to 0.***e-9 and 0.0**e-9 respectively. The training progress is terminated after the stop criteria is reached.

After the training process, the weighs and biases of the neural network are output as the constant model parameters. Thus, the coefficients of the POD representation can be predicted for any given strain sequence, which is followed by the computing of the Cauchy stress sequence. The tangent matrix and the residual vector of the finite element formulation are derived using the symbolic differentiation tool AceGen. 

Firstly, the 2D POD-FNN based plasticity model is tested by a tapered cantilever beam clamped at the left end, also known as the Cook's membrane problem. The beam is loaded at the right end by a constant distributed vertical load $q_0=0.03$, as depicted in Fig.\ref{cookgeo2D}. In this study, the quadratic finite element with 9 nodes is employed. The geometric domain of the structure is discretized by 40 quadratic 9-node quadrilateral elements with 189 nodes.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.4\columnwidth}
	\import{chap_MachineLearning/}{cookgeo.pdf_tex}
	\caption{2D cook's membrane problem.}
	\label{cookgeo2D}
\end{figure}

The final deformation state of the beam with neural network based plasticity model (NN model) is compared with that using the classical plasticity model, which are depicted in Fig.\ref{cook2D}. It can be observed that the vertical displacement of the structure is quilt close for the two models.\\

\begin{figure}[!htb]
	\centering
	\subfigure[With plasticity model]{\label{cookj2}\includegraphics[width=75mm]{chap_MachineLearning/cook_plas.jpg}}
	\subfigure[With NN model]{\label{cookrnn}\includegraphics[width=75mm]{chap_MachineLearning/cook_plasFNNPOD.jpg}}
	\caption{Final deformation state of the 2D cook's membrane.}
	\label{cook2D}
\end{figure}
The load displacement curve of the upper node $(48, 60)$ at the right end of the cantilever beam, is plotted in Fig.\ref{cookUL}. The figure shows a good agreement between the two models.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{cook2D-uf.pdf_tex}
	\caption{Load deflection curve of the 2D cook's membrane.}
	\label{cookUL}
\end{figure}

The second example to test the POD-FNN based plasticity model is a punch test as shown in Fig.\ref{punchgeo2D}, where the vertical displacement boundary condition $(u_0=0.15)$ is imposed on the top of the block and the bottom of the block is only fix in the vertical direction. The block is discretized with 100 quadratic 9-node quadrilateral elements with 441 nodes.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.5\columnwidth}
	\import{chap_MachineLearning/}{punch.pdf_tex}
	\caption{2D punch problem.}
	\label{punchgeo2D}
\end{figure}
The final deformation state of the block with neural network based plasticity model is compared with that using the classical plasticity model, which are depicted in Fig.\ref{punch2D}. It can be observed that the horizontal displacement of the structure is quite close for the two models.\\

\begin{figure}[!htb]
	\centering
	\subfigure[With plasticity model]{\label{beamj2}\includegraphics[width=70mm]{chap_MachineLearning/punch_plas.jpg}}
	\qquad
	\subfigure[With NN model]{\label{beamnn}\includegraphics[width=70mm]{chap_MachineLearning/punch_plasNN.jpg}}
	\caption{Final deformation state of the 2D block.}
	\label{punch2D}
\end{figure}

The load displacement curve of the upper node $(0, 1)$ at the left end of the block is plotted in Fig.\ref{punchUL}, where it can be seen that the neural network based model follows the plasticity model quite well except the small oscillations at the end of loading.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{punch2D-uf.pdf_tex}
	\caption{Load deflection curve of the 2D punch problem.}
	\label{punchUL}
\end{figure}

\subsubsection{Applications in 3D finite element analysis}
In this section, the machine learning based elasto-plasticity model will be evaluated in 3D. To generate the training data, one hexahedron finite element is applied under the loading condition of the tension and compression described in section 7.3.3. The von Mises plasticity with a exponential isotropic hardening law $\sigma_y = y_0+y_0(0.00002+\gamma)^{0.1}$ is set as the target model. The material parameters are set as Young's modulus $E=10$, Poison's ratio $\nu=0.33$, and the initial yield stress $y_0=0.3$. During the training data preparation, the strain-stress sequences along 8100 loading paths are generated based on the description in Fig.\ref{path-sphere}, where 90 values are assigned to the angle $\phi$ and $\theta$ respectively. Then the coefficient sequences corresponding to the stress sequences are computed by the POD.

In 3D case, three neural networks are required to predict the three coefficients of the POD representation, which are corresponding to the three principle Cauchy stress components. The same network architecture (6-20-20-1) is employed for the three feed forward neural networks. The three total strain components together with the three accumulated absolute strains are applied as the input of the neural networks. The output of the neural network is the coefficient. 

During the training, the Levenberg-Marquardt algorithm is applied as the training algorithm. After 2000 epochs of training for each neural networks, the mean squared errors are decreased to 0.0**e-9, 0.1e-9 and 0.00e-9 respectively. The training progress is terminated after the maximum epoch is reached. After the training, the POD-FNN based model is implemented in the FEM framework.

The first example to test the 3D POD-FNN based plasticity model is the necking of a bar as shown in Fig.\ref{bar3Dgeo}, where the left end of the bar is fixed and the right end is imposed a displacement boundary $u_0=1$ along its axial direction. An artificial imperfection is set in the in the center of the bar to trigger the necking, where the radius at the center is chosen to be $R_c= 0.98R$. The bar is discretized with 200 quadratic 27-node elements with 2193 nodes.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{bar3Dgeo.pdf_tex}
	\caption{Geometry and boundary conditions of the bar.}
	\label{bar3Dgeo}
\end{figure}

Fig.\ref{bar3D} shows the final deformation of the bar after tension, where only one quarter of the bar is computed due to the symmetry, it can be observed that the amounts of the necking computed by the two models are close to each other.\\

\begin{figure}[!htb]
	\centering
	\subfigure[With plasticity model]{\label{plas}\includegraphics[width=120mm]{chap_MachineLearning/bar3D.jpg}}
	\qquad\\
	\subfigure[With NN model]{\label{nn}\includegraphics[width=120mm]{chap_MachineLearning/bar3DNN.jpg}}
	\caption{Final deformation state of cylindrical bar.}
	\label{bar3D}
\end{figure}

The load displacement curve of the bar under  uniaxial tension loading is plotted in Fig.\ref{bar3D-uf}. It can be the neural network based model follows the plasticity model quite well.\\
\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{bar3D-uf.pdf_tex}
	\caption{Load deflection curve of the bar.}
	\label{bar3D-uf}
\end{figure}

The second example to test the 3D NN based plasticity model is the punch test, where the vertical displacement boundary condition $(u_0=0.15)$ is imposed on the top of the block and the bottom of the block is only fix in the vertical direction, as shown in Fig.\ref{punchgeo3D}. The block is discretized with 100 quadratic 27-node elements with 441 nodes.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.5\columnwidth}
	\import{chap_MachineLearning/}{punch3Dgeo.pdf_tex}
	\caption{2D punch problem.}
	\label{punchgeo3D}
\end{figure}

Fig.\ref{punch3D} shows the final deformation of the block after compression. It can be observed that the displacements in the horizontal direction computed by the two models are close to each other.\\

\begin{figure}[!htb]
	\centering
	\subfigure[With plasticity model]{\label{punch3D}\includegraphics[width=75mm]{chap_MachineLearning/punch3D.jpg}}
	\subfigure[With NN model]{\label{barnn}\includegraphics[width=75mm]{chap_MachineLearning/punch3D.jpg}}
	\caption{Final deformation state of the 3D block.}
	\label{punch3D}
\end{figure}

The load displacement curve of the block under compression is plotted in Fig.\ref{punch3D-uf}. It can be the neural network based model follows the plasticity model quite well.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{punch3D-uf.pdf_tex}
	\caption{Load deflection curve of the 3D block.}
	\label{punch3D-uf}
\end{figure}

The last example to test the 3D neural network based model is the Cook's membrane problem of a tapered cantilever beam, clamped at the left end. The 3D beam is loaded at the right end by a constant distributed vertical load $q_0=0.03$, as depicted in Fig.\ref{cookgeo3D}. By use of the quadratic finite element with 27 nodes, the beam is discretized with 1080 elements with 10309 nodes.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.5\columnwidth}
	\import{chap_MachineLearning/}{cook3Dgeo.pdf_tex}
	\caption{3D cook's membrane problem.}
	\label{cookgeo3D}
\end{figure}

Fig.\ref{cook3D} shows the final deformation of the block after compression. It can be observed that the displacements in the vertical direction computed by the two models are close to each other.\\

\begin{figure}[!htb]
	\centering
	\subfigure[With plasticity model]{\label{a}\includegraphics[width=70mm]{chap_MachineLearning/cook3D.jpg}}
	\qquad 
	\subfigure[With NN model]{\label{cook3DNN}\includegraphics[width=70mm]{chap_MachineLearning/cook3DNN.jpg}}
	\caption{Final deformation state of the 3D cook's membrane.}
	\label{cook3D}
\end{figure}

The load displacement curve of the block under compression is plotted in Fig.\ref{cook3D-uf}. It can be the neural network based model follows the plasticity model quite well.\\

\begin{figure}[!htb]
	\centering
	\def\svgwidth{0.7\columnwidth}
	\import{chap_MachineLearning/}{cook3D-uf.pdf_tex}
	\caption{Load deflection curve of the 3D cook's membrane.}
	\label{cook3D-uf}
\end{figure}

